Incompressibility of H-free edge modification problems: Towards a dichotomy

Given a graph $G$ and an integer $k$, the $H$-free Edge Editing problem is to find whether there exists at most $k$ pairs of vertices in $G$ such that changing the adjacency of the pairs in $G$ results in a graph without any induced copy of $H$. The existence of polynomial kernels for $H$-free Edge Editing received significant attention in the parameterized complexity literature. Nontrivial polynomial kernels are known to exist for some graphs $H$ with at most 4 vertices, but starting from 5 vertices, polynomial kernels are known only if $H$ is either complete or empty. This suggests the conjecture that there is no other $H$ with at least 5 vertices were $H$-free Edge Editing admits a polynomial kernel. Towards this goal, we obtain a set $\mathcal{H}$ of nine 5-vertex graphs such that if for every $H\in\mathcal{H}$, $H$-free Edge Editing is incompressible and the complexity assumption $NP \not\subseteq coNP/poly$ holds, then $H$-free Edge Editing is incompressible for every graph $H$ with at least five vertices that is neither complete nor empty. That is, proving incompressibility for these nine graphs would give a complete classification of the kernelization complexity of $H$-free Edge Editing for every $H$ with at least 5 vertices. We obtain similar result also for $H$-free Edge Deletion. Here the picture is more complicated due to the existence of another infinite family of graphs $H$ where the problem is trivial (graphs with exactly one edge). We obtain a larger set $\mathcal{H}$ of nineteen graphs whose incompressibility would give a complete classification of the kernelization complexity of $H$-free Edge Deletion for every graph $H$ with at least 5 vertices. Analogous results follow also for the $H$-free Edge Completion problem by simple complementation.

==> churn/old/c-claw.tex <==
\begin{lemma}
  \label{lem:c-claw}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that $H - V_\ell$ is a complete graph and $H-V_h$ is a claw. 
\end{lemma}
\begin{proof}
  Clearly, $|V_m|\leq 2$. Let $\{v_1,v_2,v_3,v_4\}$ induces the claw ($H-V_h$), where $v_1$ is the degree-3 vertex in the claw. 
  
  Case 1: $V_m=\emptyset$. Clearly $\ell\geq 3$. Then the graph is 3-connected.
  
  Case 2: $V_m$ contains $v_1$. Then the degree of $v_1$ is at least $h$, a contradiction.
  
  Case 3: $V_m=\{v_2\}$. Then $\ell\geq 3$. Then $H$ is 3-connected, a contradiction. 
\end{proof}

\begin{corollary}
  \label{cor:clawb-is}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that $H - V_\ell$ is a $\overline{\text{claw}}$ and $H-V_h$ is an empty graph. 
\end{corollary}

==> churn/old/c-diamond.tex <==
\begin{lemma}
  \label{lem:c-diamond}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that $H - V_\ell$ is a complete graph and $H-V_h$ is a diamond. 
\end{lemma}
\begin{proof}
  If $V_m=\emptyset$, then $\ell\geq 3$ and $H$ is 3-connected, a contradiction. If $V_m$ contains a degree-3 vertex of the diamond, then the degree of it is at least $h$, a contradiction. Therefore, assume that $V_m$ does not contain a degree-3 vertex of the diamond. If $V_m$ contains a degree-2 vertex, then every vertex in $V_h$ is adjacent to all vertices in the diamond, and there are vertices with different degrees in $V_\ell$, a contradiction.
\end{proof}

\begin{corollary}
  \label{cor:diamondb-is}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that $H - V_\ell$ is a $\overline{\text{diamond}}$ and $H-V_h$ is an empty graph. 
\end{corollary}

==> churn/old/c-p3.tex <==
\begin{lemma}
  \label{lem:c-p3}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that $H - V_\ell$ is a complete graph and $H-V_h$ is a $P_3$. 
\end{lemma}
\begin{proof}
  The constraints imply that $0\leq |V_m|\leq 2$. Let the vertices of the $P_3$ induced by $H-V_h$ be $\{v_1,v_2,v_3\}$ where $v_2$ is the degree-2 vertex in the $P_3$. 
  
  Let $V_m=\emptyset$. Clearly, $\ell\geq 2$. Since every vertex in $V_h$ is adjacent to equal number of vertices in $V_\ell$, we obtain that $3\ell-4 = t|V_h|$, where $t$ is the number of neighbors in $V_\ell$ of every vertex in $V_h$. If $\ell=2$, then $t=1$ and $H$ is a $C_5$, a contradiction. If $\ell\geq 3$, then $H$ is 3-connected, a contradiction. 
  If $V_m$ contains $v_2$, then $b$ has degree at least $h$, a contradiction. Therefore, assume that $V_m$ does not contain $v_2$. If $V_m=\{v_1\}$, then every vertex in $V_h$ is adjacent to all vertices in $V_\ell$ and then $v_2$ has degree at least $h$, a contradiction.
\end{proof}

\begin{corollary}
  \label{cor:p3b-is}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that $H - V_\ell$ is a $\overline{P_3}$ and $H-V_h$ is an empty graph. 
\end{corollary}



==> churn/old/c-paw.tex <==
\begin{lemma}
  \label{lem:c-paw}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that $H - V_\ell$ is a complete graph and $H-V_h$ is a paw. 
\end{lemma}
\begin{proof}
  If $V_m=\emptyset$, then $\ell\geq 3$ and $H$ is 3-connected. If $V_m$ contains the degree-3 vertex of the paw, then degree of it is at least $h$, a contradiction. Therefore, assume that $V_m$ does not contain the degree-3 vertex of the paw. If $V_m$ contains a degree-2 vertex of a paw, then every vertex in $h$ is adjacent to every vertex of the paw and the degree-3 vertex of the paw (which belongs to $V_\ell$) has degree at least $h$, a contradiction. If $V_m$ contains the degree-1 vertex of the paw, then $H$ is 3-connected, a contradiction.  
\end{proof}

\begin{corollary}
  \label{cor:pawb-is}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that $H - V_\ell$ is a $\overline{\text{paw}}$ and $H-V_h$ is an empty graph. 
\end{corollary}

==> churn/old/claw-c.tex <==
\begin{lemma}
  \label{lem:claw-c}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that  $H-V_\ell$ is a claw and $H-V_h$ is a complete graph.
\end{lemma}
\begin{proof}
  Let $V(H)\setminus V_\ell$ be $\{v_1, v_2, v_3, v_4\}$, which induces a claw in $H$, where $v_1$ is the center of the claw. 
  Since $V_\ell\cup V_m$ induces a clique, the following cases are to be analysed.

  Case 1: $V_m=\emptyset$:
  For every vertex $v$ in $V_\ell$, there are $t$ edges between $v$ and $V_h$, for some $t\geq 0$.
  If $t=0$, then $V_h$ contains vertices with different degrees, a contradiction.
  If $t=1$, then $v_2, v_3$, and $v_4$ must be adjacent to all vertices in $V_\ell$, which is a 
  contradiction (as $t=1$). If $t\geq 2$, $\ell$ is greater than deg$(v_2)$, a contradiction.

  Case 2: $v_1\in V_m$:
  Since $v_1$ is a universal vertex, degree of a vertex in $V_h$ cannot be more than that of $v_1$, a contradiction.

  Case 3: $V_m=\{v_2\}$:
  Since degree of $v_2$ is $|V_\ell|+1$ and $\ell = |V_\ell|$, there are no edges between $V_\ell$ and $V_h$. Then $V_h$ contains vertices with
  different degrees, a contradiction.
\end{proof}

\begin{corollary}
  \label{cor:claw-c}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that $H-V_\ell$ is an empty graph and $H-V_h$ is $\overline{\text{claw}}$ graph.
\end{corollary}



==> churn/old/claw-claw.tex <==
\begin{lemma}
  \label{lem:claw-claw}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is claw, and
  \item $H-V_h$ is claw.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:clawb-clawb}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{\text{claw}}$, and
  \item $H-V_h$ is $\overline{\text{claw}}$.
  \end{itemize}
\end{corollary}



==> churn/old/claw-clawb.tex <==
\begin{lemma}
  \label{lem:claw-clawb}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is claw, and
  \item $H-V_h$ is $\overline{\text{claw}}$.
  \end{itemize}
\end{lemma}




==> churn/old/claw-diamond.tex <==
\begin{lemma}
  \label{lem:claw-diamond}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is claw, and
  \item $H-V_h$ is diamond.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:diamondb-clawb}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{\text{diamond}}$, and
  \item $H-V_h$ is $\overline{\text{claw}}$.
  \end{itemize}
\end{corollary}



==> churn/old/claw-diamondb.tex <==
\begin{lemma}
  \label{lem:claw-diamondb}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is claw, and
  \item $H-V_h$ is $\overline{\text{diamond}}$.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:diamond-clawb}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is diamond, and
  \item $H-V_h$ is $\overline{\text{claw}}$.
  \end{itemize}
\end{corollary}



==> churn/old/claw-is.tex <==

\begin{lemma}
  \label{lem:claw-is}
  Let $H\notin \mathcal{X}\cup \mathcal{Y}$ be such that $H-V_\ell$ is a claw and $H-V_h$ is an empty graph.
  Then $H$ is \dominatedby\ $H_2$.
\end{lemma}
\begin{proof}
  Let $V(H)\setminus V_\ell$ be $\{v_1, v_2, v_3, v_4\}$, which induces a claw, where $v_1$ is the center of the claw.
  Since $V_\ell\cup V_m$ induces an independent set, the following cases are to be analysed.

  Case 1: $V_m=\emptyset$:
  Since vertices in $V_h$ must have the same degree, $\ell\geq 1$.
  A degree counting gives us that $\ell|V_\ell| = 4h-6$.
  If $\ell =1$ or $\ell=2$, $\overline{H}$ is 3-connected, a contradiction.
  If $\ell\geq 3$, then $H$ is 3-connected, a contradiction. 

  Case 2: $V_m=\{v_1\}$:
  Since deg$(v_1)=3$, we obtain that $h\geq 4$, $\ell\geq 1$, and a degree counting gives us $\ell|V_\ell|= 3(h-1)$. If $\ell=1$, then $|V_\ell|=3(h-1)$ and
  we obtain that $\overline{H}$ is 3-connected, a contradiction. If $\ell=2$, then $|V_\ell|=3/2(h-1)$ and $\overline{H}$ is 
  3-connected, a contradiction. If $\ell\geq 3$, $H$ is 3-connected, a contradiction.

  Case 3: $V_m=\{v_2\}$: Since deg$(v_2)=1$, $\ell=0$. Then $V_h$ has vertices with different degrees, a contradiction.

  Case 4: $V_m=\{v_2, v_3\}$: Since deg$(v_2)=$ deg$(v_3)=1$, $\ell = 0$. Then $V_h$ has vertices with different degrees, a contradiction.

  Case 5: $V_m=\{v_2, v_3, v_4\}$: Since vertices in $V_\ell$ must have degree less that of vertices in $V_m$, $\ell=0$. Then $H$ is claw $\cup tK_1$, for some $t\geq 1$.
  Then $H$ can be reduced to $H_2$ (claw $\cup K_1$) (Corollary~\ref{cor:jutk1}). 
\end{proof}

\begin{corollary}
  \label{cor:c-clawb}
  Let $H\notin \mathcal{X}\cup \mathcal{Y}$ be such that $H-V_\ell$ is a complete graph and $H-V_h$ is $\overline{\text{claw}}$.
  Then $H$ is \dominatedby\ $H_2$.
\end{corollary}


==> churn/old/claw-p3.tex <==
\begin{lemma}
  \label{lem:claw-p3}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is claw, and
  \item $H-V_h$ is $P_3$.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:p3b-clawb}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{P_3}$, and
  \item $H-V_h$ is $\overline{\text{claw}}$.
  \end{itemize}
\end{corollary}



==> churn/old/claw-p4.tex <==
\begin{lemma}
  \label{lem:claw-p4}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is claw, and
  \item $H-V_h$ is $P_4$.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:p4-clawb}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $P_4$, and
  \item $H-V_h$ is $\overline{\text{claw}}$.
  \end{itemize}
\end{corollary}



==> churn/old/claw-paw.tex <==
\begin{lemma}
  \label{lem:claw-paw}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is claw, and
  \item $H-V_h$ is paw.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:pawb-clawb}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{\text{paw}}$, and
  \item $H-V_h$ is $\overline{\text{claw}}$.
  \end{itemize}
\end{corollary}



==> churn/old/claw-pawb.tex <==
\begin{lemma}
  \label{lem:claw-pawb}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is claw, and
  \item $H-V_h$ is $\overline{\text{paw}}$.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:paw-clawb}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is paw, and
  \item $H-V_h$ is $\overline{\text{claw}}$.
  \end{itemize}
\end{corollary}



==> churn/old/clawb-claw.tex <==
\begin{lemma}
  \label{lem:clawb-claw}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{\text{claw}}$, and
  \item $H-V_h$ is claw.
  \end{itemize}
\end{lemma}




==> churn/old/clawb-diamond.tex <==
\begin{lemma}
  \label{lem:clawb-diamond}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{\text{claw}}$, and
  \item $H-V_h$ is diamond.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:dimondb-claw}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{\text{diamond}}$, and
  \item $H-V_h$ is claw.
  \end{itemize}
\end{corollary}



==> churn/old/clawb-paw.tex <==
\begin{lemma}
  \label{lem:clawb-paw}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{\text{claw}}$, and
  \item $H-V_h$ is paw.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:pawb-claw}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{\text{paw}}$, and
  \item $H-V_h$ is claw.
  \end{itemize}
\end{corollary}



==> churn/old/diamond-c.tex <==
%Before getting into the case in which $H-V_\ell$ is a diamond and $H-V_h$ is a complete graph, we need to following lemma.
\begin{comment}
\begin{lemma}
  \label{lem:diamond-special}
  Let $H$ (see Figure~\ref{fig:z671}) be a graph on 6 vertices $\{v_1, v_2, v_3, v_4, v_5, v_6\}$ and 7 edges such that $\{v_1, v_2, v_3, v_4\}$ induces a $C_4$ where $\{v_1, v_3\}$ forms a 
  pair of nonadjacent vertices and $\{v_2, v_5, v_6, v_4\}$ induces $P_4$ where $v_2$ and $v_4$ are the end vertices. Then $H$ is reducible to $C_4$.
\end{lemma}
\begin{proof}
  Let $H'$ be the $C_4$ induced by $V'= \{v_1,v_2,v_3,v_4\}$.
  Let $(G',k)$ be an instance of \HDEE. Construct $G$ from $(G',k, H, V')$ by Construction~\ref{con:main}. We claim that $(G',k)$ is a yes-instance 
  of \HDEE\ if and only if $(G,k)$ is a yes-instance of \HEE. 

  Let $(G',k)$ be a yes-instance with a solution $F'$. We claim that $G\triangle F'$ is $H$-free. For a contradiction, assume that $G\triangle F'$
  has an induced $H$. Since a vertex introduced during the construction cannot be any of $\{v_1, v_2, v_3, v_4\}$, $G'\triangle F'$ has an induced $C_4$,
  which is a contradiction. Proposition~\ref{pro:con:main-backward} proves the other direction.
\end{proof}
\end{comment}
\begin{lemma}
  \label{lem:diamond-c}
  Let $H\notin \mathcal{X}\cup \mathcal{Y}$ be such that $H-V_\ell$ is a diamond and $H-V_h$ is a complete graph.
  Then $H$ can be reduced to $H'\in \{C_4, A_1\}$.
\end{lemma}
\begin{proof}
  Let $V(H)\setminus V_\ell$ be $\{v_1, v_2, v_3, v_4\}$, which induces a diamond in $H$, where $v_1, v_2$ be the vertices with degree 3 and $v_3, v_4$ be the 
  vertices with degree 2 in the induced diamond. 
  Since $V_\ell\cup V_m$ induces a clique, the following cases are to be analysed.

  Case 1: $V_m=\emptyset$:
  For every vertex $v$ in $V_\ell$, there are $t$ edges between $v$ and $V_h$, for some $t\geq 0$. We observe that $h\geq 3$.
  If $t=0$, then $V_h$ contains vertices with different degrees, a contradiction.
  If $t=1$ and $h=3$, then $\overline{H}$ (see Figure~\ref{fig:z671}) can be reduced to $C_4$ (Corollary~\ref{cor:path}). If $t=1$ and $h\geq 4$, then $H$ is 
  3-connected, a contradiction. If $t=2$ and $h=3$, then $H$ is $\overline{A_1}$. If $t=2$ and $h\geq 4$, then $H$ is 3-connected,
  a contradiction. If $t\geq 3$, then $H$ is 3-connected, a contradiction.

  Case 2: $v_1\in V_m$: Since $v_1$ is a universal vertex, vertices in $V_h$ have degree at most that of $v_1$, a contradiction.

  Case 3: $V_m=\{v_3\}$:
  Since deg$(v_3)=|V_\ell|+2$, deg$(v_4)$ cannot exceed that of $v_3$, a contradiction.
\end{proof}

\begin{lemma}
  \label{cor:diamond-c}
  Let $H\notin \mathcal{X}\cup \mathcal{Y}$ be such that $H-V_\ell$ is an empty graph and $H-V_h$ is $\overline{\text{diamond}}$.
  Then $H$ can be reduced to $H'\in\{C_4, A_1\}$.
\end{lemma}


==> churn/old/diamond-claw.tex <==
\begin{lemma}
  \label{lem:diamond-claw}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is diamond, and
  \item $H-V_h$ is claw.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:clawb-diamondb}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{\text{claw}}$, and
  \item $H-V_h$ is $\overline{\text{diamond}}$.
  \end{itemize}
\end{corollary}




==> churn/old/diamond-diamond.tex <==
\begin{lemma}
  \label{lem:diamond-diamond}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is diamond, and
  \item $H-V_h$ is diamond.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:diamondb-diamondb}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{\text{diamond}}$, and
  \item $H-V_h$ is $\overline{\text{diamond}}$.
  \end{itemize}
\end{corollary}




==> churn/old/diamond-diamondb.tex <==
%It can be verified that there are four graphs $H$ satisfying the conditions in Lemma~\ref{lem:diamond-diamondb} which are pairs of graphs which are complements to each other.
%One pair can be reduced to the other pair using Corollary~\ref{cor:path1}, and the other pair can be reduced to $\overline{H_{10}}$ (Corollary~\ref{cor:jutk1}).
\begin{lemma}
  \label{lem:diamond-diamondb}
  Let $H\notin \mathcal{X}\cup \mathcal{Y}$ be such that 
  \begin{itemize}
  \item $H-V_\ell$ is diamond, and
  \item $H-V_h$ is $\overline{\text{diamond}}$.
  \end{itemize}
  Then $H$ can be reduced to $H_{10}$.
\end{lemma}



==> churn/old/diamond-is.tex <==
\begin{comment}
Before resolving the case of $H-V_h$ being a diamond and $H-V_h$ being an empty graph, we need the following lemma.
\begin{lemma}
  \label{lem:diamond-special2}
  Let $H$ be a graph on 7 vertices $v_1, v_2\ldots v_{7}$ and 10 edges such that $\{v_1,v_2,v_3\}$ induces a triangle, $\{v_1, v_6, v_7\}$ induces a triangle,
  and $\{v_2, v_3, v_4, v_5\}$ induces a diamond, where $v_4$ and $v_5$ are nonadjacent. Then $H$ is \dominatedby\ $\overline{H_4}$. 	
\end{lemma}
\begin{proof}
  Let $V'$ be $\{v_1,v_2,v_3,v_4,v_5\}$. Let $H'$ be $\overline{H_4}$ induced by $V'$. Let $(G,k)$ be an instance of \HDEE. We construct $G$ from $(G',k,H,V')$ by 
  Construction~\ref{con:main}. We claim that $(G',k)$ is an yes-instance of \HDEE\ if and only if $(G,k)$ is a yes-instance of \HEE.

  Let $(G,k)$ be a yes-instance and let $F'$ be a solution. We claim that $G\triangle F'$ is $H$-free. For a contradiction assume that $G\triangle F'$
  has an induced $H$. We observe that none of the vertices introduced during the construction can act as a vertex in $V'$ in the induced $H$. Therefore,
  $G'\triangle F'$ has an induced $H'$, which is a contradiction. Proposition~\ref{pro:con:main-backward} proves the other direction.
\end{proof}
\end{comment}

\begin{lemma}
  \label{lem:diamond-is}
  Let $H\notin \mathcal{X}\cup \mathcal{Y}$ be such that $H-V_\ell$ is a diamond and $H-V_h$ is an empty graph.
  Then there exists an $H'\in \{H_4, H_{6}, H_7, H_{8}, A_1, A_{9}\}$ 
  such that $H$ is \dominatedby\ $H'$.
\end{lemma}
\begin{proof}
  Let $H-V_\ell$ be $\{v_1, v_2, v_3, v_4\}$ which induces a diamond, where $v_1$ and $v_2$ are the vertices with degree 3 in the induced diamond.
  Since $V_\ell\cup V_m$ is an independent set, the following cases are to be analysed.

  Case 1: $V_m=\emptyset$: Clearly, $\ell\geq 1$ and $h\geq 3$. If $\ell=1$ and $h=3$, then $H$ is $A_{9}$. If $\ell=1$ and $h\geq 4$, 
  then $\overline{H}$ is 3-connected, a contradiction. If $\ell=2$ and $h=3$, then $H$ is $\overline{A_1}$. If $\ell=2$ and $h=4$,
  then either $H$ is the complement of the graph shown in Figure~\ref{fig:7101} (in this case the graph is \dominatedby\ $\overline{H_4}$ - Corollary~\ref{cor:path}) 
  or $H$ is the graph shown in Figure~\ref{fig:z7111} which is \dominatedby\ $\overline{A_{1}}$ (Corollary~\ref{cor:mod}). 
  If $\ell=2$ and $h=5$, either $\overline{H}$ is 3-connected or $H$ is the graph shown in Figure~\ref{fig:z9151}, which is \dominatedby\ the graph shown in Figure~\ref{fig:z7111} (Corollary~\ref{cor:mod}), which is \dominatedby\ $\overline{A_1}$ (Corollary~\ref{cor:mod}). 
  If $\ell=2$ and 
  $h > 5$, then $\overline{H}$ is 3-connected, a contradiction. If $\ell\geq 3$, then $H$ is 3-connected, a contradiction.

  Case 2: $V_m=\{v_1\}$: Since deg$(v_1)=3$, $\ell\leq 2$ and $h\geq 4$. If $\ell=0$, $V_h$ has vertices with different degrees, a contradiction.
  If $\ell=1$, $\overline{H}$ is 3-connected, a contradiction. If $\ell=2$, then there exists no $H$ with $h=4$. If $\ell=2$ and $h=5$, then $H$
  is the graph shown in Figure~\ref{fig:z8131} which
  is \dominatedby\ $\overline{A_1}$ (Corollary~\ref{cor:mod}). If $\ell=2$ and $h\geq 6$, then $\overline{H}$ (if exists) is 3-connected, a contradiction.

  Case 3: $V_m=\{v_3\}$. Since deg$(v_3)=2$, $\ell\leq 1$ and $h\geq 3$. If $\ell=0$, $V_h$ has vertices with different degrees, a contradiction.
  If $\ell=1$ and $h=3$, then $H$ is $\overline{H_7}$. If $\ell=1$ and $h\geq 4$, then $\overline{H}$ is 3-connected, a contradiction.

  Case 4: $V_m=\{v_3, v_4\}$. Since deg$(v_3)=$ deg$(v_4)=2$, $\ell\leq 1$ and $h\geq 3$. If $\ell=0$ and $h=3$, then $H$ is diamond $\cup tK_1$ for some
  $t\geq 1$. Then $H$ is \dominatedby\ $\overline{H_{8}}$ (Corollary~\ref{cor:jutk1}). There exist no $H$ with $\ell=0$ and $h\geq 4$. If $\ell = 1$, then $h\geq 4$.
  If $\ell=1$ and $h=4$, then $H$ is the complement of the graph shown in Figure~\ref{fig:c671} which is \dominatedby\ $H_6$ (Lemma~\ref{lem:h12}). If $\ell=1$ and $h=5$, then $H$ is the graph shown in Figure~\ref{fig:z891} which is \dominatedby\ the complement of the graph shown in Figure~\ref{fig:c671} (Corollary~\ref{cor:mod}) which is \dominatedby\ $H_6$ (Lemma~\ref{lem:h12}). 
  If $\ell=1$ and $h\geq 6$,
  then $\overline{H}$ is 3-connected, a contradiction.  
\end{proof}

\begin{corollary}
  \label{cor:c-diamondb}
  Let $H\notin \mathcal{X}\cup \mathcal{Y}$ be such that $H-V_\ell$ is a complete graph and $H-V_h$ is $\overline{\text{diamond}}$ graph.
  Then there exists an $H'\in \{H_4, H_{6}, H_7, H_{8}, A_1, A_{9}\}$ 
  such that $H$ is \dominatedby\ $H'$.
\end{corollary}



==> churn/old/diamond-p3.tex <==
\begin{lemma}
  \label{lem:diamond-p3}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is diamond, and
  \item $H-V_h$ is $P_3$.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:p3b-diamondb}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{P_3}$, and
  \item $H-V_h$ is $\overline{\text{diamond}}$.
  \end{itemize}
\end{corollary}




==> churn/old/diamond-p4.tex <==
\begin{lemma}
  \label{lem:diamond-p4}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is diamond, and
  \item $H-V_h$ is $P_4$.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:p4-diamondb}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $P_4$, and
  \item $H-V_h$ is $\overline{\text{diamond}}$.
  \end{itemize}
\end{corollary}




==> churn/old/diamond-paw.tex <==
\begin{lemma}
  \label{lem:diamond-paw}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is diamond, and
  \item $H-V_h$ is paw.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:pawb-diamondb}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{\text{paw}}$, and
  \item $H-V_h$ is $\overline{\text{diamond}}$.
  \end{itemize}
\end{corollary}




==> churn/old/diamondb-diamond.tex <==

\begin{lemma}
  \label{lem:diamondb-diamond}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{\text{diamond}}$, and
  \item $H-V_h$ is diamond.
  \end{itemize}
\end{lemma}



==> churn/old/is-claw.tex <==
\begin{lemma}
  \label{lem:is-claw}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that $H - V_\ell$ is an empty graph and $H-V_h$ is a claw. 
\end{lemma}
\begin{proof}
  Clearly, $|V_m|\leq 3$. Let $\{v_1,v_2,v_3,v_4\}$ induces the claw ($H-V_h$), where $v_1$ is the degree-3 vertex in the claw. If $V_m=\emptyset$, then $\ell\geq 3$ and $h\leq 4$. Then $\ell=3$ and $h=4$, which is not possible. If $V_m$ contains $v_1$, then $v_1$
  has degree at least $h$, a contradiction. If $V_m$ contains $v_2$, then the degree of $v_2$ is at most $\ell$, a contradiction. 
\end{proof}

\begin{corollary}
  \label{cor:clawb-c}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that $H - V_\ell$ is a $\overline{\text{claw}}$ and $H-V_h$ is a complete graph. 
\end{corollary}

==> churn/old/is-diamond.tex <==
\begin{lemma}
  \label{lem:is-diamond}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that $H - V_\ell$ is an empty graph and $H-V_h$ is a diamond. 
\end{lemma}
\begin{proof}
  If $V_m=\emptyset$, then $\ell\geq 3$ and $h\leq 4$. Therefore, $\ell=3$ and $h=4$ and there exists no such graph. If $V_m$ contains a degree-3 vertex of the diamond, then the degree of it is at least $h$, a contradiction. Therefore, assume that $V_m$ does not contain a degree-3 vertex of the diamond. If $V_m$ contains a degree-2 vertex of the diamond, then it has degree at most $\ell$, a contradiction.
\end{proof}

\begin{corollary}
  \label{cor:diamondb-c}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that $H - V_\ell$ is a $\overline{\text{diamond}}$ and $H-V_h$ is a complete graph. 
\end{corollary}

==> churn/old/is-p3.tex <==
\begin{lemma}
  \label{lem:is-p3}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that $H - V_\ell$ is an  empty graph and $H-V_h$ is a $P_3$. 
\end{lemma}
\begin{proof}
  Clearly, $|V_m|\leq 2$. Let $\{v_1,v_2,v_3\}$ induced the $P_3$ ($H-V_h$), where $v_2$ is the degree-2 vertex in the $P_3$. 
  
  Let $V_m=\emptyset$. Clearly $\ell\geq 2$ and $h\leq 3$. Therefore, $\ell=2$ and $h=3$. Then every vertex in $V_h$ is adjacent to every vertex in $V_\ell$. This is a contradiction as vertices in $V_\ell$ get different degrees. If $V_m$ contains $v_2$, then the degree of it is at least $h$, which is a contradiction. If $V_m$ contains either $v_1$ or $v_3$ or both, then the degree of them is at most $\ell$, which is a contradiction.
\end{proof}

\begin{corollary}
  \label{cor:p3b-c}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that $H - V_\ell$ is a $\overline{P_3}$ and $H-V_h$ is a complete graph. 
\end{corollary}

==> churn/old/is-paw.tex <==
\begin{lemma}
  \label{lem:is-paw}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that $H - V_\ell$ is an empty graph and $H-V_h$ is a paw. 
\end{lemma}
\begin{proof}
  If $V_m=\emptyset$, then $\ell\geq 3$ and $h\leq 4$. Therefore, $\ell=3$ and $h=4$ but then a vertex in $V_\ell$ gets a degree at least four, a contradiction.
  If $V_m$ contains the degree-3 vertex of the paw, then the degree of it is at least $h$, a contradiction. Therefore, assume that $V_m$ does not contain that vertex. If $V_m$ contains a degree-2 vertex of the paw, then $\ell\geq h$, a contradiction. If $V_m$ contains just the degree-1 vertex of the paw, then it has degree at most $\ell$, a contradiction.
\end{proof}

\begin{corollary}
  \label{cor:pawb-c}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that $H - V_\ell$ is a $\overline{\text{paw}}$ and $H-V_h$ is a complete graph. 
\end{corollary}

==> churn/old/p3-c.tex <==

\begin{lemma}
  \label{lem:p3-c}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that $H-V_\ell$ is a $P_3$ and $H-V_h$  is a complete graph.
\end{lemma}
\begin{proof}
  Let $\{v_1, v_2, v_3\}$ be the set $V(H)\setminus V_\ell$ which induces a $P_3$ where $v_2$ 
  be the degree-2 vertex of the $P_3$. If $|V_\ell|=1$, then $|V(H)|=4$, a contradiction. Therefore, 
  $|V_\ell|\geq 2$.

  Case 1: $V_m=\emptyset$

  This implies that $V_\ell$ induces a clique and $V_h=\{v_1,v_2,v_3\}$ induces a $P_3$.
  To make sure that vertices in $V_h$ have degree more than $\ell$, there must be edges
  from $v_1$ and $v_3$ to all vertices in $V_\ell$. This gives a contradiction as $v_1$ and 
  $v_2$ have degree at most $\ell$.

  Case 2: $V_m\neq \emptyset$

  Then, without loss of generality, we can assume that $V_m=\{v_1\}$, $V_m=\{v_2\}$ or $V_m=\{v_1,v_2\}$.

  Case 2a: $V_m=\{v_1\}$

  Since $V_\ell\cup V_m$ forms a clique, to make sure that every vertex in $V_\ell$ has degree $\ell$ which is
  greater than that of $v_1$, none of the vertices in $V_\ell$ can have edges to $v_2$ or $v_3$. Then $\ell=|V_\ell|\geq 2$.
  Thus we get a contradiction as deg$(v_3)=1<\ell$.

  Case 2b: $V_m=\{v_2\}$ or $V_m=\{v_1,v_2\}$

  Since $v_2$ is a universal vertex, $v_3$ cannot have degree more than that of $v_2$, a contradiction.
\end{proof}

\begin{corollary}
  \label{cor:is-p3b}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that $H-V_\ell$ is an empty graph and $H-V_h$ is a $\overline{P_3}$.
\end{corollary}



==> churn/old/p3-claw.tex <==
\begin{lemma}
  \label{lem:p3-claw}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $P_3$, and
  \item $H-V_h$ is claw.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:clawb-p3b}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{\text{claw}}$, and
  \item $H-V_h$ is $\overline{P_3}$.
  \end{itemize}
\end{corollary}



==> churn/old/p3-clawb.tex <==
\begin{lemma}
  \label{lem:p3-clawb}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $P_3$, and
  \item $H-V_h$ is $\overline{\text{claw}}$.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:claw-p3b}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is claw, and
  \item $H-V_h$ is $\overline{P_3}$.
  \end{itemize}
\end{corollary}



==> churn/old/p3-diamond.tex <==
\begin{lemma}
  \label{lem:p3-diamond}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $P_3$, and
  \item $H-V_h$ is diamond.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:diamondb-p3b}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{\text{diamond}}$, and
  \item $H-V_h$ is $\overline{P_3}$.
  \end{itemize}
\end{corollary}



==> churn/old/p3-diamondb.tex <==
It can be verified that the only graph satisfying the conditions in Lemma~\ref{lem:p3-diamondb} is $P_5\cup P_2$ which can be reduced to $P_5$ by Proposition~\ref{pro:disconnected}.
\begin{lemma}
  \label{lem:p3-diamondb}
  Let $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $P_3$, and
  \item $H-V_h$ is $\overline{\text{diamond}}$.
  \end{itemize}
  Then $H$ can be reduced to $P_5$.
\end{lemma}

\begin{corollary}
  \label{cor:diamond-p3b}
  Let $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is diamond, and
  \item $H-V_h$ is $\overline{P_3}$.
  \end{itemize}
  Then $H$ can be reduced to $P_5$.
\end{corollary}



==> churn/old/p3-is.tex <==
\begin{lemma}
  \label{lem:p3-is}
  Let $H\notin \mathcal{X}\cup \mathcal{Y}$ be such that $H-V_\ell$ is a $P_3$ and $H-V_h$ is an empty graph.
  Then there exists an $H'\in \{C_4, H_1\}$ such that $H$ is \dominatedby\ $H'$.
\end{lemma}
\begin{proof}
  Let $\{v_1,v_2,v_3\}$ be $H-V_\ell$ which induces a $P_3$ where $v_2$ be the vertex with degree two in the $P_3$.
  Clearly, $\ell\leq 3$ and $|V_\ell|\geq 2$. 
  Since $H-V_h$ is an empty graph, the following cases are to be analysed.
  
  Case 1: $V_m=\emptyset$: Then $1\leq \ell\leq 3$.
  A degree counting yields $\ell|V_\ell| = 3h-4$. 
  Case 1a: $\ell = 3$: Then we get that vertices in $V_h$ have different degrees, a contradiction.
  Case 1b: $\ell = 2$: In this case we get that $|V_\ell| = 3h/2 - 2$ and hence $h > 2$ is a multiple of 2. If $h=4$ then $|V_\ell|=4$
  and $H$ is the graph shown in Figure~\ref{fig:z7101} which is \dominatedby\ $C_4$ (Corollary~\ref{cor:mod}). 
  If $h\geq 6$ then we obtain that $\overline{H}$ is 3-connected, 
  a contradiction.
  Case 1c: $\ell=1$: Then $H$ is either $P_5$ or 3-connected, both are contradictions.

  Case 2: $V_m=\{v_1\}$: Since $V_\ell\cup V_m$ is an independent set, $v_1$ has degree 1. Therefore, $\ell=0$. Then we get deg$(v_3)$ is same as 
  that of $v_1$, which is a contradiction.

  Case 3: $V_m=\{v_2\}$: Then $h\geq 3$ and $\ell=1$. Then $\overline{H}$ is 3-connected, a contradiction.

  Case 4: $V_m=\{v_1, v_3\}$: Since $V_\ell\cup V_m$ is an independent set, $v_1$ and $v_2$ have degree 1 in $H$.
  Therefore $\ell=0$. Therefore, $H$ is $P_3\cup tK_1$ for some $t\geq 2$. If $t\geq 3$, $\overline{H}$ is 3-connected, a contradiction.
  If $t=2$, $H$ is $H_1$.
\end{proof}


\begin{corollary}
  \label{cor:c-p3b}
  Let $H\notin \mathcal{X}\cup \mathcal{Y}$ be such that $H-V_\ell$ is a complete graph and $H-V_h$ is $\overline{P_3}$.
  Then there exists an $H'\in \{C_4, H_1\}$ such that $H$ is \dominatedby\ $H'$.
\end{corollary}



==> churn/old/p3-p3.tex <==
\begin{lemma}
  \label{lem:p3-p3}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $P_3$, and
  \item $H-V_h$ is $P_3$.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:p3b-p3b}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{P_3}$, and
  \item $H-V_h$ is $\overline{P_3}$.
  \end{itemize}
\end{corollary}


==> churn/old/p3-p3b.tex <==
\begin{lemma}
  \label{lem:p3-p3b}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $P_3$, and
  \item $H-V_h$ is $\overline{P_3}$.
  \end{itemize}
\end{lemma}



==> churn/old/p3-p4.tex <==
\begin{lemma}
  \label{lem:p3-p4}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $P_3$, and
  \item $H-V_h$ is $P_4$.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{lem:p4-p3b}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $P_4$, and
  \item $H-V_h$ is $\overline{P_3}$.
  \end{itemize}
\end{corollary}



==> churn/old/p3-paw.tex <==
\begin{lemma}
  \label{lem:p3-paw}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $P_3$, and
  \item $H-V_h$ is paw.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{lem:pawb-p3b}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{\text{paw}}$, and
  \item $H-V_h$ is $\overline{P_3}$.
  \end{itemize}
\end{corollary}



==> churn/old/p3-pawb.tex <==
\begin{lemma}
  \label{lem:p3-pawb}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $P_3$, and
  \item $H-V_h$ is $\overline{paw}$.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{lem:paw-p3b}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is paw, and
  \item $H-V_h$ is $\overline{P_3}$.
  \end{itemize}
\end{corollary}



==> churn/old/p3b-claw.tex <==
\begin{lemma}
  \label{lem:p3b-claw}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{P_3}$, and
  \item $H-V_h$ is claw.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:clawb-p3}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{\text{claw}}$, and
  \item $H-V_h$ is $P_3$.
  \end{itemize}
\end{corollary}



==> churn/old/p3b-diamond.tex <==
\begin{lemma}
  \label{lem:p3b-diamond}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{P_3}$, and
  \item $H-V_h$ is diamond.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:diamondb-p3}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{\text{diamond}}$, and
  \item $H-V_h$ is $P_3$.
  \end{itemize}
\end{corollary}



==> churn/old/p3b-p3.tex <==
\begin{lemma}
  \label{lem:p3b-p3}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{P_3}$, and
  \item $H-V_h$ is $P_3$.
  \end{itemize}
\end{lemma}



==> churn/old/p3b-paw.tex <==
\begin{lemma}
  \label{lem:p3b-paw}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{P_3}$, and
  \item $H-V_h$ is paw.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:pawb-p3}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{\text{paw}}$, and
  \item $H-V_h$ is $P_3$.
  \end{itemize}
\end{corollary}



==> churn/old/p4-c.tex <==
\begin{lemma}
  \label{lem:p4-c}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that $H-V_\ell$ is a $P_4$ and $H-V_h$ is a complete graph.
\end{lemma}
\begin{proof}
  Let $V(H)-V_\ell$ be $\{v_1,v_2, v_3, v_4\}$ which induces a $P_4$, where $v_1$ and $v_4$ are the end vertices and
  $v_2$ is adjacent to $v_1$, and $v_3$ is adjacent to $v_4$. 
  Since $V_\ell\cup V_m$ induces a clique, the following cases are to be analysed.

  Case 1: $V_m=\emptyset$: Every vertex in $V_\ell$ is adjacent to $t$ vertices in $V_h$, for some $t\geq 0$.
  If $t=0$, $V_h$ has vertices with different degrees, a contradiction. If $t=1$, then $\ell = |V_\ell|$, and $v_1$
  and $v_4$ must be adjacent to all vertices in $V_\ell$ (as $h>\ell$). This gives a contradiction as $t=1$.
  If $t\geq 2$ $v_1$ and $v_4$ will have degree $\ell$, a contradiction. 

  Case 2: $V_m = \{v_1\}$: Since $V_\ell\cup V_m$ induces a clique, $v_1$ has degree $|V_\ell|+1$ and $\ell=|V_\ell|$. None of $v_2, v_3$, and $v_4$ can 
  have edges to $V_\ell$. This gives a contradiction as $v_3$ and $v_4$ have different degrees.

  Case 3: $v_2\in V_m$: Since $V_\ell\cup V_m$ induces a clique, $v_2$ has degree $|V_\ell|+2$ and none of the vertices in $V_h$ can obtain 
  a degree more than this, a contradiction.
\end{proof}

\begin{corollary}
  \label{cor:p4-c}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that $H-V_\ell$ is an empty graph and $H-V_h$ is a $P_4$.
\end{corollary}




==> churn/old/p4-claw.tex <==
\begin{lemma}
  \label{lem:p4-claw}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $P_4$, and
  \item $H-V_h$ is claw.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{lem:clawb-p4}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{\text{claw}}$, and
  \item $H-V_h$ is $P_4$.
  \end{itemize}
\end{corollary}



==> churn/old/p4-diamond.tex <==
\begin{lemma}
  \label{lem:p4-diamond}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $P_4$, and
  \item $H-V_h$ is diamond.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:diamondb-p4}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{\text{diamond}}$, and
  \item $H-V_h$ is $P_4$.
  \end{itemize}
\end{corollary}



==> churn/old/p4-is.tex <==
\begin{lemma}
  \label{lem:p4-is}
  Let $H\notin \mathcal{X}\cup \mathcal{Y}$ be such that  $H-V_\ell$ is a $P_4$ and $H-V_h$ is an empty graph.
  Then $H$ is \dominatedby\ $H_4$.
\end{lemma}
\begin{proof}
  Let $V(H)-V_\ell$ be $\{v_1,v_2, v_3, v_4\}$ which induces a $P_4$, where $v_1$ and $v_4$ are the end vertices and
  $v_2$ is adjacent to $v_1$, and $v_3$ is adjacent to $v_4$.
  Since $V_\ell\cup V_m$ induces an empty graph, the following cases are to be considered.

  Case 1: $V_m = \emptyset$: 
  Since $V_h$ induces a $P_4$, and every vertex in $V_h$ has degree $h$, $\ell\geq 1$. 
  If $\ell = 1$, then $h\geq 2$ and $\overline{H}$ is 3-connected, a contradiction.
  If $\ell=2$, then $|V_\ell| = 2h-3$ and $\overline{H}$ is 3-connected, a contradiction.
  If $\ell\geq 3$, then $H$ is 3-connected, a contradiction.

  Case 2: $v_1\in V_m=\{v_1\}$: Since vertices in $V_\ell$ must have degree less than that of $v_1$, $\ell=0$.
  Then $v_3$ and $v_4$ are having different degrees, a contradiction.

  Case 3: $V_m=\{v_2\}$: Since degree of $v_2$ is 2, $\ell$ is either 0 or 1 and $h\geq 3$. If $\ell=0$, we get a contradiction similar to the previous case.
  If $\ell=1$, then $\overline{H}$ is 3-connected, a contradiction.

  Case 4: $V_m=\{v_1,v_4\}$: Then $\ell=0$, $h=2$, and $H$ is $P_4\cup tK_1$ for some $t\geq 1$. If $t=1$, then $H$ is $H_4$. If $t\geq 2$, $H$
  is \dominatedby\ $H_4$ (Corollary~\ref{cor:jutk1}).

  Case 5: $V_m=\{v_1, v_3\}$: Then, due to the degree constraints, $\ell = 0$. Then $v_2\in V_h$ and $v_3\in V_m$ have the same degree, which is 
  a contradiction.
\end{proof}

\begin{corollary}
  \label{cor:c-p4}
  Let $H\notin \mathcal{X}\cup \mathcal{Y}$ be such that  $H-V_\ell$ is a complete graph and $H-V_h$ is a $P_4$.
  Then $H$ is \dominatedby\ $H_4$.
\end{corollary}



==> churn/old/p4-p3.tex <==
\begin{lemma}
  \label{lem:p4-p3}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $P_4$, and
  \item $H-V_h$ is $P_3$.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:p3b-p4}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{P_3}$, and
  \item $H-V_h$ is $P_4$.
  \end{itemize}
\end{corollary}



==> churn/old/p4-p4.tex <==
\begin{lemma}
  \label{lem:p4-p4}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $P_4$, and
  \item $H-V_h$ is $P_4$.
  \end{itemize}
\end{lemma}



==> churn/old/p4-paw.tex <==
\begin{lemma}
  \label{lem:p4-paw}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $P_4$, and
  \item $H-V_h$ is paw.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:pawb-p4}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{\text{paw}}$, and
  \item $H-V_h$ is $P_4$.
  \end{itemize}
\end{corollary}



==> churn/old/paw-c.tex <==
\begin{lemma}
  \label{lem:paw-c}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that $H-V_\ell$ is a paw and $H-V_h$ is a complete graph.
\end{lemma}
\begin{proof}
  Let $V(H)\setminus V_\ell$ be $\{v_1, v_2, v_3, v_4\}$, which induces a paw in $H$, where $v_1$ be the vertex with degree 3, $v_2, v_3$ be the 
  vertices with degree 2, and $v_4$ be the vertex with degree 1 in the induced paw. 
  Since $V_\ell\cup V_m$ induces a clique, the following cases are to be analysed.

  Case 1: $V_m=\emptyset$:
  For every vertex $v$ in $V_\ell$, there are $t$ edges between $v$ and $V_h$, for some $t\geq 0$.
  If $t=0$, then $V_h$ contains vertices with different degrees, a contradiction.
  If $t=1$, then $v_4$ must be adjacent to all vertices in $V_\ell$. Then there cannot be 
  any other edges from $V_\ell$ to $V_h$. Then $V_h$ contains vertices with different degrees, a contradiction. 
  If $t\geq 2$, then $\ell$ is greater than deg$(v_4)$, a contradiction.

  Case 2: $v_1\in V_m$:
  Since $v_1$ is a universal vertex, degree of a vertex in $V_h$ cannot be more than that of $v_1$, a contradiction.

  Case 3: $V_m=\{v_2\}$:
  Since degree of $v_2$ is $|V_\ell|+2$. Then $h\geq |V_\ell|+3$. Since $V(H)=|V_\ell|+4$, $h=|V_\ell|+3$. Then $v_1$ has edges to all vertices in $V_\ell$.
  Then $\ell=|V_\ell|+1$. Then $V_h$ contains vertices with different degrees, a contradiction.

  Case 4: $V_m=\{v_4\}$: Since deg$(v_4)=|V_\ell|+1$, $\ell = |V_\ell|$ and there is no edge between $V_\ell$ and $V_h$. Then $V_h$ 
  contains vertices with different degrees, a contradiction.

  Case 5: $V_m=\{v_2,v_3\}$: Since deg$(v_2)=$deg$(v_3)=|V_\ell|+2$ and $\ell=|V_\ell|+1$, there is no edge between $V_\ell$ and $V_h$.
  Then $V_h$ contains vertices with different degrees, a contradiction.
\end{proof}

\begin{corollary}
  \label{cor:is-pawb}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that $H-V_\ell$ is an empty graph and $H-V_h$ is $\overline{\text{paw}}$.
\end{corollary}



==> churn/old/paw-claw.tex <==
\begin{lemma}
  \label{lem:paw-claw}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is paw, and
  \item $H-V_h$ is claw.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:clawb-pawb}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{\text{claw}}$, and
  \item $H-V_h$ is $\overline{\text{paw}}$.
  \end{itemize}
\end{corollary}



==> churn/old/paw-diamond.tex <==
\begin{lemma}
  \label{lem:paw-diamond}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is paw, and
  \item $H-V_h$ is diamond.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:diamondb-pawb}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{\text{diamond}}$, and
  \item $H-V_h$ is $\overline{\text{paw}}$.
  \end{itemize}
\end{corollary}




==> churn/old/paw-diamondb.tex <==

\begin{lemma}
  \label{lem:paw-diamondb}
  Let $H\notin \mathcal{X}\cup \mathcal{Y}$ be such that 
  \begin{itemize}
  \item $H-V_\ell$ is paw, and
  \item $H-V_h$ is $\overline{\text{diamond}}$.
  \end{itemize}
  Then $H$ is either $H_{13}$ or $H_{14}$.
\end{lemma}

\begin{corollary}
  \label{cor:diamond-pawb}
  Let $H\notin \mathcal{X}\cup \mathcal{Y}$ be such that 
  \begin{itemize}
  \item $H-V_\ell$ is diamond, and
  \item $H-V_h$ is $\overline{\text{paw}}$.
  \end{itemize}
  Then $H$ is either $\overline{H_{13}}$ or $\overline{H_{14}}$.
\end{corollary}



==> churn/old/paw-is.tex <==
\begin{lemma}
  \label{lem:paw-is}
  Let $H\notin \mathcal{X}\cup \mathcal{Y}$ be such that $H-V_\ell$ is a paw and $H-V_h$ is an empty graph.
  Then $H$ is \dominatedby\ an $H'\in \{H_6, A_{4}\}$.
\end{lemma}
\begin{proof}
  Let $H-V_\ell=\{v_1, v_2, v_3, v_4\}$, which induces a paw in $H$, where $v_1$ be the vertex with degree 3, $\{v_2,v_3\}$ be vertices with degree 2,
  and $v_4$ be the vertex with degree 1 in the induced paw. Since $V_\ell\cup V_m$ is an independent set, we have the following cases to be analysed.

  Case 1: $V_m=\emptyset$: A simple degree counting gives us $\ell|V_\ell| = 4h-8$. Further, $\ell\geq 1$ and $h\geq 3$. 
  
  Case 1a: $\ell=1$: Then $|V_\ell| = 4h-8$ and $\overline{H}$
  is 3-connected, a contradiction. 

  Case 1b: $\ell=2$: Then $V_\ell=2h-4$. If $h=3$, $H$ is $\overline{A_{4}}$. If $h\geq 4$, $\overline{H}$ is 3-connected.

  Case 1c: $\ell\geq 3$: Then $H$ is 3-connected, a contradiction.

  Case 2: $V_m=\{v_1\}$: Since deg$(v_1)=3$, $\ell\leq 2$ and $h\geq 4$. If $\ell=0$, $V_h$ has vertices with different degrees, a contradiction.
  If $\ell=1$ or $\ell=2$, $\overline{H}$ is 3-connected, a contradiction.

  Case 3: $V_m=\{v_2\}$: Since deg$(v_2)=2$, $\ell\leq 1$ and $h\geq 3$. If $\ell=0$, $V_h$ has vertices with different degrees, a contradiction.
  If $\ell = 1$, then $\overline{H}$ is 3-connected, a contradiction.

  Case 4: $V_m=\{v_4\}$. Since deg$(v_4)=1$, $\ell=0$ and there cannot be any edge between $V_\ell$ and $V_h$. Then $V_h$ has vertices with
  different degrees, a contradiction.

  Case 5: $V_m=\{v_2, v_4\}$: Since deg$(v_2)=2$ and deg$(v_4)=1$, we obtain that $\ell=0$ and $h\geq 3$. Since there is no edge between $V_\ell$
  and $V_h$, $h=3$. Then $H$ is paw $\cup tK_1$, for any $t\geq 1$. Then $H$ can be reduced to paw $\cup K_1$ ($H_6$) (Corollary~\ref{cor:jutk1}). 
\end{proof}


\begin{corollary}
  Let $H\notin \mathcal{X}\cup \mathcal{Y}$ be such that $H-V_\ell$ is a complete graph and $H-V_h$ is $\overline{\text{paw}}$.
  Then $H$ can be reduced to some $H'\in \{H_6, A_{4}\}$.
\end{corollary}


==> churn/old/paw-p3.tex <==
\begin{lemma}
  \label{lem:paw-p3}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is paw, and
  \item $H-V_h$ is $P_3$.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:p3b-pawb}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{P_3}$, and
  \item $H-V_h$ is $\overline{\text{paw}}$.
  \end{itemize}
\end{corollary}



==> churn/old/paw-p4.tex <==
\begin{lemma}
  \label{lem:paw-p4}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is paw, and
  \item $H-V_h$ is $P_4$.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:p4-pawb}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $P_4$, and
  \item $H-V_h$ is $\overline{\text{paw}}$.
  \end{itemize}
\end{corollary}



==> churn/old/paw-paw.tex <==
\begin{lemma}
  \label{lem:paw-paw}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is paw, and
  \item $H-V_h$ is paw.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{cor:pawb-pawb}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{\text{paw}}$, and
  \item $H-V_h$ is $\overline{\text{paw}}$.
  \end{itemize}
\end{corollary}



==> churn/old/paw-pawb.tex <==
\begin{lemma}
  \label{lem:paw-pawb}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is paw, and
  \item $H-V_h$ is $\overline{\text{paw}}$.
  \end{itemize}
\end{lemma}



==> churn/old/pawb-diamond.tex <==
\begin{lemma}
  \label{lem:pawb-diamond}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{paw}$, and
  \item $H-V_h$ is diamond.
  \end{itemize}
\end{lemma}

\begin{corollary}
  \label{lem:diamondb-paw}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{diamond}$, and
  \item $H-V_h$ is paw.
  \end{itemize}
\end{corollary}



==> churn/old/pawb-paw.tex <==
\begin{lemma}
  \label{lem:pawb-paw}
  There exists no $H\notin \mathcal{X}\cup \mathcal{Y}$ such that 
  \begin{itemize}
  \item $H-V_\ell$ is $\overline{\text{paw}}$, and
  \item $H-V_h$ is paw.
  \end{itemize}
\end{lemma}



==> figs/tiny/c5.tex <==
\fbox{\begin{tikzpicture}[myv/.style={circle, draw, inner sep=1.5pt}]
  \node (z) at (0,0) {};

  \node[myv] (a) at (54:0.43) {};
  \node[myv] (b) at (126:0.43) {};
  \node[myv] (c) at (198:0.43) {};
  \node[myv] (d) at (270:0.43) {};
  \node[myv] (e) at (342:0.43) {};

  \draw (a) -- (b);
  \draw (b) -- (c);
  \draw (c) -- (d);
  \draw (d) -- (e);
  \draw (a) -- (e);
\end{tikzpicture}}


==> tables/old/biglist-class.tex <==
%\begin{tabu}
\begin{landscape}
%\scalebox{0.75}{
\begin{longtabu}{|N|X[c]|X[c]|m{2cm}|X[c]|X[c]|X[c]|m{2.5cm}|m{2.5cm}|}%
\hline
\multicolumn{1}{|c|}{\textbf{Row}}& \textbf{$H$} & \textbf{$\overline{H}$} & \textbf{Comment} & \textbf{$H-V_\ell$} & \textbf{$H-V_h$} & \textbf{Simulates} & \textbf{Comment} & \textbf{Proved by}\\\hline
\endhead
\label{t:k2t} & $K_{2,t}$ & $K_t\cup K_2$ & $4\leq t$ & $2K_1$ & $tK_1$ & $K_{1,t}$ & see row \ref{t:k1t} & Corollary \ref{cor:jukt}, \ref{cor:folklore}\\\hline%1
\label{t:k1t} & $K_{1,t}$ & $K_t\cup K_1$ & $5\leq t$ & $K_1$ & $tK_1$ & $K_{1,4}$ & $H_5$ & Corollary \ref{cor:k1t}\\\hline%2
\label{t:k2vtk1} & $K_2\vee tK_1$ & $K_t\cup 2K_1$ & $4\leq t$ & $K_2$ & $tK_1$ & $K_2\vee 3K_1$ & $\overline{H_3}$ & Corollary \ref{cor:k2xsk1}\\\hline%3
\label{t:st1} & $S_{t,1}$ & $\overline{S_{t,1}}$ & $4\leq t$ & $K_2$ & $K_2\cup tK_1$ & $K_{1,t}$ & $H_5$ & Corollary \ref{cor:twin-star}\\\hline%4
\label{t:kt-eu2k1} & $\overline{(K_t-e)\cup 2K_1}$ & $(K_t-e)\cup 2K_1$ & $4\leq t$ & $K_4$ & $K_2\cup (t-2)K_1$ & $\overline{(K_t-e)\cup K_1}$ & see $\overline{H_8}$, $D_2$, row 8 & Corollary \ref{cor:jutk1}, \ref{cor:folklore}\\\hline%5
\label{t:kt-euk2} & $\overline{(K_t-e)\cup K_2}$ & $(K_t-e)\cup K_2$ & $4\leq t$& diamond & $K_2\cup (t-2)K_1$ & $\overline{(K_t-e)\cup K_1}$ & see $H_8$, $D_2$, row 8& Corollary \ref{cor:jukt}, \ref{cor:folklore}\\\hline%6
\label{t:k1tuk2} & $K_{1,t}\cup K_2$ & $\overline{K_{1,t}\cup K_2}$ & $4\leq t$ & $K_1$ & $K_2\cup tK_1$ & $K_{1,t}$ & see row \ref{t:k1t} & Lemma \ref{lem:disconnected}\\\hline%7
\label{t:kt-euk1} & $\overline{(K_t-e)\cup K_1}$ & $(K_t-e)\cup K_1$ & $6\leq t$ & $K_3$ & $K_2\cup (t-2)K_1$ & $K_{1,t-2}$ & see row \ref{t:k1t} & Lemma \ref{lem:near-uni-kt-euk1}\\\hline%8
\label{t:jt} & $J_t$ & $\overline{J_t}$ & $3\leq t$, see Corollary \ref{cor:path-k2vtk1} & $K_2$ & $K_2\cup tK_1$ & $K_2\vee tK_1$ & see row \ref{t:k2vtk1} & Corollary \ref{cor:path-k2vtk1}\\\hline%9
\label{t:qt} & $Q_t$ & $\overline{Q_t}$ & $3\leq t$, see Corollary \ref{cor:path-k2-t} & $2K_1$ & $K_2\cup tK_1$ & $K_{2,t}$ & see row \ref{t:k2t} and row \ref{t:k23} & Corollary \ref{cor:path-k2-t}\\\hline%10
\caption{Some infinite sets of graphs $H$ satisfying the property that $H\notin \mathcal{X}\cup \mathcal{Y}$ and $H-V_\ell$, $H-V_h\in \mathcal{Y}$}
\label{table:biglist-class}
\end{longtabu}%}
\end{landscape}
%\end{tabu}

==> tables/old/biglist-large.tex <==
%\begin{tabu}
\begin{landscape}
%\scalebox{0.75}{
\begin{longtabu}{|N|X[c]|X[c]|m{2cm}|X[c]|X[c]|X[c]|X[c]|m{3cm}|}%
\hline
\multicolumn{1}{|c|}{\textbf{Row}}& \textbf{$H$} & \textbf{$\overline{H}$} & \textbf{Comment} & \textbf{$H-V_\ell$} & \textbf{$H-V_h$} & \textbf{Simulates} & \textbf{Comment} & \textbf{Proved by}\\\hline
\endhead
\label{t:z10181} & \input{figs/large/z10181} & \input{figs/large/z10181c} & Figure \ref{fig:z10181} & $K_4$ & $7K_1$ & \input{figs/gang/c791} & $\overline{A_{9}}$ & Corollary \ref{cor:mod}\\[-2ex]\hline%1
\label{t:z11221} & \input{figs/large/z11221} & \input{figs/large/z11221c} & Figure \ref{fig:z11221} & $K_5$ & $K_2\cup 6K_1$ & \input{figs/gang/c521} & $\overline{H_{1}}$ & Corollary~\ref{cor:mod}, \ref{cor:near-uni}\\[-2ex]\hline%2
\label{t:z10231} & \input{figs/large/z10231} & \input{figs/large/z10231c} & Figure \ref{fig:z10231} & $K_6$ & $K_2\cup 4K_1$ & \input{figs/gang/542} & $H_6$ & Corollary \ref{cor:mod}, \ref{cor:folklore}, \ref{cor:near-uni}\\[-2ex]\hline%3
\label{t:z10232} & \input{figs/large/z10232} & \input{figs/large/z10232c} & Figure \ref{fig:z10232} & $K_6$ & $K_2\cup 4K_1$ & \input{figs/gang/542} & $H_6$ & Corollary \ref{cor:near-uni}, \ref{cor:folklore}, Proposition~\ref{pro:high-low}\\\hline%4
\label{t:z11341} & \input{figs/large/z11341} & \input{figs/large/z11341c} & $\overline{H}$ in Figure \ref{fig:z11341c} & $K_8$ & $K_2\cup 3K_1$ & \input{figs/gang/521} & $H_3$ & Corollary \ref{cor:mod}, \ref{cor:folklore}, \ref{cor:near-uni}, Proposition \ref{pro:high-low}\\\hline%5
\label{t:z10221c} & \input{figs/large/z10221c} & \input{figs/large/z10221} & $\overline{H}$ in Figure \ref{fig:z10221} & $K_4$ & $K_2\cup 4K_1$ & \input{figs/gang/541} & $H_5$ & Corollary \ref{cor:mod}, \ref{cor:folklore}, Lemma \ref{lem:disconnected}\\\hline%6
\label{t:z11281c} & \input{figs/large/z11281c} & \input{figs/large/z11281} & $\overline{H}$ is Figure \ref{fig:z11281} & $K_5$ & $K_2\cup 5K_1$ & \input{figs/gang/541} & $H_5$ & Corollary \ref{cor:mod} \ref{cor:folklore}, \ref{cor:k1t}, Lemma \ref{lem:disconnected}\\\hline%7
\label{t:z12281} & \input{figs/large/z12281} & \input{figs/large/z12281c} & Figure \ref{fig:z12281} & diamond & $K_2\cup 6K_1$ & \input{figs/gang/543} & $H_7$ & Lemma \ref{lem:z12281}, Corollary \ref{cor:near-uni}\\\hline%8
\caption{All graphs $H$ with at least ten vertices, except those given in Table~\ref{table:biglist-class}, such that $H\notin \mathcal{X}\cup \mathcal{Y}$ and $H-V_\ell$, $H-V_h\in \mathcal{Y}$}
\label{table:biglist-large}
\end{longtabu}%}
\end{landscape}
%\end{tabu}




==> tables/old/biglist-small.tex <==
\begin{landscape}
%\begin{small}
%\scalebox{0.75}{
\begin{longtabu}{|N|X[c]|X[c]|m{2cm}|X[c]|X[c]|X[c]|X[c]|m{2.5cm}|}%
\hline
\multicolumn{1}{|c|}{\textbf{Row}}& \textbf{$H$} & \textbf{$\overline{H}$} & \textbf{Comment} & \textbf{$H-V_\ell$} & \textbf{$H-V_h$} & \textbf{Simulates} & \textbf{Comment} & \textbf{Proved by}\\\hline
\endhead
\label{t:k23} & \input{figs/small/k23} & \input{figs/small/k23c} & $K_{2,3}$ & {$2K_1$} & {$3K_1$} & \input{figs/tiny/c4} & {$C_4$} & {Lemma~\ref{lem:k23}}\\\hline%1
\label{t:c651} & \input{figs/small/c651} & \input{figs/small/651} & Figure \ref{fig:c651} & {$K_4$} & {$K_2$} & \input{figs/gang/c543} & $\overline{H_7}$ & Corollary \ref{cor:near-uni}\\\hline%2
\label{t:c671} & \input{figs/small/c671} & \input{figs/small/671} & {Figure \ref{fig:c671}} & {$K_4$} & {$\overline{\text{diamond}}$} & \input{figs/gang/542} & {$H_6$} & {Corollary \ref{cor:near-uni}}\\\hline%3
\label{t:claw-2k1} & \input{figs/small/claw-2k1} & \input{figs/small/claw-2k1c} & $\text{claw}\cup 2K_1$ & claw & $5K_1$ & \input{figs/gang/531} & $H_2$ & Corollary \ref{cor:jutk1}\\\hline%4
\label{t:z671} & \input{figs/small/z671} & \input{figs/small/z671c} & Figure \ref{fig:z671} & $2K_1$ & $\overline{\text{diamond}}$ & \input{figs/tiny/c4} & $C_4$ & Corollary \ref{cor:path}\\\hline%5
\label{t:paw-2k1} & \input{figs/small/paw-2k1} & \input{figs/small/paw-2k1c} & $\text{paw}\cup 2K_1$ & paw & $K_2\cup 3K_1$ & \input{figs/gang/542} & $H_6$ & Corollary \ref{cor:jutk1}\\\hline%6
\label{t:z771} & \input{figs/small/z771} & \input{figs/small/z771c} & Figure \ref{fig:z771} & $K_3$ & $5K_1$ & \input{figs/gang/552} & $H_9$ & Corollary \ref{cor:mod}\\[-2ex]\hline%7
\label{t:z7111} & \input{figs/small/z7111} & \input{figs/small/z7111c} & Figure \ref{fig:z7111} & diamond & $3K_1$ & \input{figs/gang/c532} & $\overline{A_1}$ & Corollary \ref{cor:mod}\\\hline%8
\label{t:z7102} & \input{figs/small/z7102} & \input{figs/small/z7102c} & Figure \ref{fig:z7102} & $K_3$ & $\overline{\text{diamond}}$ & \input{figs/gang/c534} & $\overline{H_4}$ & Corollary \ref{cor:path}\\[-2ex]\hline%9
\label{t:z7101} & \input{figs/small/z7101} & \input{figs/small/z7101c} & Figure \ref{fig:z7101} & $P_3$ & $4K_1$ & \input{figs/tiny/c4} & $C_4$ & Corollary \ref{cor:mod}\\\hline%10
\label{t:z781} & \input{figs/small/z781} & \input{figs/small/z781c} & Figure \ref{fig:z781} & diamond & $K_2\cup 3K_1$ & \input{figs/gang/c543} & $\overline{H_7}$ & Corollary \ref{cor:path-k2-t}\\\hline%11
\label{t:z8141} & \input{figs/small/z8141} & same & Figure \ref{fig:z8141} & $K_4$ & $4K_1$ & \input{figs/gang/c543} & $\overline{H_7}$ & Corollary \ref{cor:mod}, \ref{cor:near-uni}\\[-2ex]\hline%12
\label{t:z8101} & \input{figs/small/z8101} & \input{figs/small/z8101c} & Figure \ref{fig:z8101} & $K_4$ & $K_2\cup 4K_1$ & \input{figs/small/c671} & see row \ref{t:c671} & Corollary \ref{cor:mod}\\[-2ex]\hline%13
\label{t:z8151c} & \input{figs/small/z8151c} & \input{figs/small/z8151} & $\overline{H}$ in Figure~\ref{fig:z8151} & $K_4$ & $K_2\cup 3K_1$ & \input{figs/gang/clawuk2} & $B_1$ & Corollary \ref{cor:mod}, \ref{cor:folklore}\\\hline%14
\label{t:z8132} & \input{figs/small/z8132} & \input{figs/small/z8132c} & Figure~\ref{fig:z8132} & $K_4$ & $K_2\cup 3K_1$ & \input{figs/gang/552} & $H_9$ & Corollary \ref{cor:path}, Lemma~\ref{lem:disconnected}\\\hline%15
\label{t:z8133} & \input{figs/small/z8133} & \input{figs/small/z8133c} & Figure~\ref{fig:z8133} & $K_5$ & $K_2\cup 3K_1$ & \input{figs/small/c671} & see row \ref{t:c671} & Corollary \ref{cor:near-uni}\\[-2ex]\hline%16
\label{t:z8122c} & \input{figs/small/z8122c} & \input{figs/small/z8122} & Figure \ref{fig:z8122c} & $K_5$ & $K_2\cup 3K_1$ & \input{figs/gang/c521} & $\overline{H_1}$ & Corollary \ref{cor:near-uni}\\[-2ex]\hline%17
\label{t:z8131} & \input{figs/small/z8131} & \input{figs/small/z8131c} & Figure \ref{fig:z8131} & diamond & $5K_1$ & \input{figs/gang/c532} & $\overline{A_1}$ & Corollary \ref{cor:mod}\\[-2ex]\hline%18
\label{t:z891} & \input{figs/small/z891} & \input{figs/small/z891c} & Figure \ref{fig:z891} & diamond & $6K_1$ & \input{figs/small/671} & see row \ref{t:c671} & Corollary \ref{cor:mod}\\[-2ex]\hline%19
\label{t:z8171c} & \input{figs/small/z8171c} & \input{figs/small/z8171} & {Figure \ref{fig:z8171c}} & {$P_3$} & {$K_2\cup 3K_1$} & \input{figs/small/k24} & {see row \ref{t:k2t}} & {Corollary \ref{cor:cut-z8171c}}\\\hline%20
\label{t:z8134} & \input{figs/small/z8134} & \input{figs/small/z8134c} & Figure \ref{fig:z8134} & diamond & $K_2\cup 3K_1$ & \input{figs/gang/c534} & $\overline{H_4}$ & Corollary \ref{cor:mod}\\[-2ex]\hline%21
\label{t:z8121} & \input{figs/small/z8121} & \input{figs/small/z8121c} & {Figure \ref{fig:z8121}} & {diamond} & {$\overline{\text{diamond}}$} & \input{figs/small/diamonduk2c} & {see row \ref{t:kt-euk2}} & {Corollary~\ref{cor:mod}}\\\hline%22
\label{t:z9211c} & \input{figs/small/z9211c} & \input{figs/small/z9211} & Figure \ref{fig:z9211c} & $K_3$ & $6K_1$ & \input{figs/gang/c663} & $\overline{A_7}$ & Corollary~\ref{cor:mod}\\[-2ex]\hline%23
\label{t:z9181} & \input{figs/small/z9181} & same & Figure \ref{fig:z9181} & $K_5$ & $5K_1$ & \input{figs/small/z771c} & see row \ref{t:z771} & Corollary~\ref{cor:mod}\\[-2ex]\hline%24
\label{t:z9161} & \input{figs/small/z9161} & \input{figs/small/z9161c} & Figure \ref{fig:z9161} & $K_4$ & $K_2\cup 4K_1$ & \input{figs/gang/c521} & $\overline{H_1}$ & Corollary~\ref{cor:mod}\\[-2ex]\hline%25
\label{t:z9151} & \input{figs/small/z9151} & \input{figs/small/z9151c} & Figure \ref{fig:z9151} & diamond & $5K_1$ & \input{figs/small/z7111} & see row \ref{t:z7111} & Corollary~\ref{cor:mod}\\[-2ex]\hline%26
\label{t:z9141} & \input{figs/small/z9141} & \input{figs/small/z9141c} & Figure \ref{fig:z9141} & diamond & $K_2\cup 4K_1$ & \input{figs/small/k5-euk2c} & see row \ref{t:kt-euk2} & Corollary~\ref{cor:cut-z9141}\\\hline%27
\caption{All graphs $H$ with at most nine vertices, except those given in Table~\ref{table:biglist-class}, such that $H\notin \mathcal{X}\cup \mathcal{Y}$ and $H-V_\ell$, $H-V_h\in \mathcal{Y}$. These are revealed by a computer search.}
\label{table:biglist-small}
\end{longtabu}%}
%\end{small}
\end{landscape}

==> tables/old/biglist.tex <==
%\begin{tabu}
\begin{landscape}
%\scalebox{0.75}{
\begin{longtabu}{|m{0.75cm}|X[c]|X[c]|m{2cm}|X[c]|X[c]|X[c]|m{2.5cm}|m{2.5cm}|}%
\hline
\textbf{Row}& \textbf{$H$} & \textbf{$\overline{H}$} & \textbf{Comment} & \textbf{$H-V_\ell$} & \textbf{$H-V_h$} & \textbf{Dom. by} & \textbf{Comment} & \textbf{Proved by}\\\hline
\endhead
1 & \input{figs/k23} & \input{figs/k23c} & $K_{2,3}$ & $2K_1$ & $3K_1$ & \input{figs/c4} & $C_4$ & Lemma~\ref{lem:k23}\\\hline
2 & $K_{2,t}$ & $K_t\cup K_2$ & $4\leq t\leq 7$ & $2K_1$ & $tK_1$ & $K_{1,t}$ & see row 3& Corollary \ref{cor:jukt}, \ref{cor:folklore}\\\hline
3 & $K_{1,t}$ & $K_t\cup K_1$ & $5\leq t\leq 8$ & $K_1$ & $tK_1$ & $K_{1,4}$ & $H_5$ & Corollary \ref{cor:k1t}\\\hline
4 & $K_2\vee tK_1$ & $K_t\cup 2K_1$ & $4\leq t\leq 7$ & $K_2$ & $tK_1$ & $K_2\vee 3K_1$ & $\overline{H_3}$ & Corollary \ref{cor:k2xsk1}\\\hline
5 & $S_{t,1}$ & $\overline{S_{t,1}}$ & $4\leq t\leq 6$ & $K_2$ & $K_2\cup tK_1$ & $K_{1,t}$ & $H_5$ & Corollary \ref{cor:twin-star}\\\hline
6 & \input{figs/c671} & \input{figs/671} & Figure \ref{fig:c671} & $K_4$ & $\overline{\text{diamond}}$ & \input{figs/542} & $H_6$ & Corollary \ref{cor:near-uni}\\\hline
7 & $\overline{(K_t-e)\cup 2K_1}$ & $(K_t-e)\cup 2K_1$ & $4\leq t\leq 7$ & $K_4$ & $K_2\cup (t-2)K_1$ & $\overline{(K_t-e)\cup K_1}$ & see $H_8$, $B_3$, row 14 & Corollary \ref{cor:jutk1}, \ref{cor:folklore}\\\hline
8 & \input{figs/claw-2k1} & \input{figs/claw-2k1c} & $\text{claw}\cup 2K_1$ & claw & $5K_1$ & \input{figs/531} & $H_2$ & Corollary \ref{cor:jutk1}\\\hline
9 & \input{figs/z671} & \input{figs/z671c} & Figure \ref{fig:z671} & $2K_1$ & $\overline{\text{diamond}}$ & \input{figs/c4} & $C_4$ & Corollary \ref{cor:path}\\\hline
10 & \input{figs/paw-2k1} & \input{figs/paw-2k1c} & $\text{paw}\cup 2K_1$ & paw & $K_2\cup 3K_1$ & \input{figs/542} & $H_6$ & Corollary \ref{cor:jutk1}\\\hline
11 & $\overline{(K_t-e)\cup K_2}$ & $(K_t-e)\cup K_2$ & $4\leq t\leq 7$& diamond & $K_2\cup (t-2)K_1$ & $\overline{(K_t-e)\cup K_1}$ & see $H_8$, $B_3$, row 14& Corollary \ref{cor:jutk1}, \ref{cor:folklore}\\\hline
12 & \input{figs/z771} & \input{figs/z771c} & Figure \ref{fig:z771} & $K_3$ & $5K_1$ & \input{figs/552} & $H_9$ & Corollary \ref{cor:mod}\\\hline
13 & $K_{1,t}\cup K_2$ & $\overline{K_{1,t}\cup K_2}$ & $4\leq t\leq 6$ & $K_1$ & $K_2\cup tK_1$ & $K_{1,t}$ & see row 3 & Lemma \ref{lem:disconnected}\\\hline
14 & $\overline{(K_t-e)\cup K_1}$ & $(K_t-e)\cup K_1$ & $6\leq t\leq 8$ & $K_3$ & $K_2\cup (t-2)K_1$ & $\overline{K_{t-2}\cup K_1}$ & see row 3 & Lemma \ref{lem:near-uni-kt-euk1}\\\hline
15 & \input{figs/z7111} & \input{figs/z7111c} & Figure \ref{fig:z7111} & diamond & $3K_1$ & \input{figs/c532} & $\overline{A_1}$ & Corollary \ref{cor:mod}\\\hline
16 & \input{figs/z7102} & \input{figs/z7102c} & Figure \ref{fig:z7102} & $K_3$ & $\overline{\text{diamond}}$ & \input{figs/c534} & $\overline{H_4}$ & Corollary \ref{cor:path}\\\hline
17 & $J_t$ & $\overline{J_t}$ & $3\leq t\leq 5$, see Corollary \ref{cor:path-k2vtk1} & $K_2$ & $K_2\cup tK_1$ & $K_2\vee tK_1$ & see row 4 & Corollary \ref{cor:path-k2vtk1}\\\hline
18 & \input{figs/z7101} & \input{figs/z7101c} & Figure \ref{fig:z7101} & $P_3$ & $4K_1$ & \input{figs/c4} & $C_4$ & Corollary \ref{cor:mod}\\\hline
19 & $Q_t$ & $\overline{Q_t}$ & $3\leq t\leq 5$, see Corollary \ref{cor:path-k2-t} & $2K_1$ & $K_2\cup tK_1$ & $K_{2,t}$ & see row 1,2 & Corollary \ref{cor:path-k2-t}\\\hline
20 & \input{figs/z781} & \input{figs/z781c} & Figure \ref{fig:z781} & diamond & $K_2\cup 3K_1$ & \input{figs/c543} & $\overline{H_7}$ & Corollary \ref{cor:path-k2-t}\\\hline
21 & \input{figs/782} & \input{figs/782c} & Figure \ref{fig:782} & diamond & $K_2\cup 3K_1$ & \input{figs/543} & $H_7$ & Corollary \ref{cor:near-uni}\\\hline
22 & \input{figs/z8141} & same & Figure \ref{fig:z8141} & $K_4$ & $4K_1$ & \input{figs/c651} & $\overline{A_2}$ & Corollary \ref{cor:mod}\\\hline
23 & \input{figs/z8101} & \input{figs/z8101c} & Figure \ref{fig:z8101} & $K_4$ & $K_2\cup 4K_1$ & \input{figs/c671} & see row 6 & Corollary \ref{cor:mod}\\\hline
24 & \input{figs/z8151c} & \input{figs/z8151} & $\overline{H}$ in Figure~\ref{fig:z8151} & $K_4$ & $K_2\cup 3K_1$ & \input{figs/clawuk2} & $B_1$ & Corollary \ref{cor:mod}, \ref{cor:folklore}\\\hline
25 & \input{figs/z8132} & \input{figs/z8132c} & Figure~\ref{fig:z8132} & $K_4$ & $K_2\cup 3K_1$ & \input{figs/552} & $H_9$ & Corollary \ref{cor:path}, Lemma~\ref{lem:disconnected}\\\hline
26 & \input{figs/z8133} & \input{figs/z8133c} & Figure~\ref{fig:z8133} & $K_5$ & $K_2\cup 3K_1$ & \input{figs/c671} & see row 6 & Corollary \ref{cor:near-uni}\\\hline
27 & \input{figs/z8122c} & \input{figs/z8122} & Figure \ref{fig:z8122c} & $K_5$ & $K_2\cup 3K_1$ & \input{figs/c521} & $\overline{H_1}$ & Corollary \ref{cor:near-uni}\\\hline
28 & \input{figs/z8131} & \input{figs/z8131c} & Figure \ref{fig:z8131} & diamond & $5K_1$ & \input{figs/c532} & $\overline{A_1}$ & Corollary \ref{cor:mod}\\\hline
29 & \input{figs/z891} & \input{figs/z891c} & Figure \ref{fig:z891} & diamond & $6K_1$ & \input{figs/671} & see row 6 & Corollary \ref{cor:mod}\\\hline
30 & \input{figs/z8171c} & \input{figs/z8171} & Figure \ref{fig:z8171c} & $P_3$ & $K_2\cup 3K_1$ & \input{figs/k24} & $K_{2,4}$, see row 2 & Corollary \ref{cor:cut-z8171c}\\\hline
31 & \input{figs/z8134} & \input{figs/z8134c} & Figure \ref{fig:z8134} & diamond & $K_2\cup 3K_1$ & \input{figs/c534} & $\overline{H_4}$ & Corollary \ref{cor:mod}\\\hline
32 & \input{figs/z8135} & \input{figs/z8135c} & $\overline{H}$ in Figure \ref{fig:z8135c} & diamond & $K_2\cup 3K_1$ & \input{figs/c534} & $\overline{H_4}$ & Lemma \ref{lem:near-uni-z8135c}, Corollary \ref{cor:folklore}\\\hline
33 & \input{figs/z8121} & \input{figs/z8121c} & Figure \ref{fig:z8135c} & diamond & $\overline{\text{diamond}}$ & \input{figs/diamonduk2c} & $\overline{\text{diamond}\cup K_2}$, see row 11 & Corollary~\ref{cor:mod}\\\hline
34 & \input{figs/z9211c} & \input{figs/z9211} & Figure \ref{fig:z9211c} & $K_3$ & $6K_1$ & \input{figs/c663} & $\overline{A_8}$ & Corollary~\ref{cor:mod}\\\hline
35 & \input{figs/z9181} & same & Figure \ref{fig:z9181} & $K_5$ & $5K_1$ & \input{figs/z771c} & see row 12 & Corollary~\ref{cor:mod}\\\hline
36 & \input{figs/z9161} & \input{figs/z9161c} & Figure \ref{fig:z9161} & $K_4$ & $K_2\cup 4K_1$ & \input{figs/c521} & $\overline{H_1}$ & Corollary~\ref{cor:mod}\\\hline
37 & \input{figs/z9151} & \input{figs/z9151c} & Figure \ref{fig:z9151} & diamond & $5K_1$ & \input{figs/z7111} & see row 15 & Corollary~\ref{cor:mod}\\\hline
38 & \input{figs/z9141} & \input{figs/z9141c} & Figure \ref{fig:z9141} & diamond & $K_2\cup 4K_1$ & \input{figs/k5-euk2c} & $\overline{(K_5-e)\cup K_2}$, see row 11 & Corollary~\ref{cor:cut-z9141}\\\hline
\caption{..}
\label{table:biglist}
\end{longtabu}%}
\end{landscape}
%\end{tabu}




==> tables/old/c-is-table.tex <==
\begin{table}
\begin{center}
\scalebox{1}{
\begin{tabular}{|c|c|c|b{2.2cm}|c|c|c|c|}\hline
Row & $H$ & $\overline{H}$ & Comment & Dominated by & Comment & Proved by\\\hline
1 & $K_{1,t}$ & $K_t\cup K_1$ & $5\leq t\leq 8$ & \input{figs/541} & $H_5$ & Corollary~\ref{cor:k1t}\\\hline
2 & $K_2\vee sK_1$ & $K_s\cup 2K_1$ & $4\leq s\leq 7$ & \input{figs/c533} & $\overline{H_3}$ & Corollary~\ref{cor:k2xsk1}\\\hline
3 & \input{figs/z9211} & \input{figs/z9211c} & See Figure~\ref{fig:z9211} & \input{figs/663} & $A_8$ & Corollary~\ref{cor:mod}, \ref{cor:folklore}\\\hline
\end{tabular}}
\end{center}
\caption{Graphs $H$ (and $\overline{H}$) shown in this table are the set of graphs with at most nine vertices such that $H-V_\ell$ is a complete graph and $H-V_\ell$ is an empty graph and and neither $H$ nor $\overline{H}$ is in $\mathcal{H}\cup\mathcal{A}\cup\mathcal{X}$. See Lemma~\ref{lem:c-is}.}
\label{table:c-is}
\end{table}

==> tables/old/cai-table.tex <==
\begin{table}
\begin{center}
\scalebox{1}{
\begin{tabular}{|l||*{6}{c|}}\hline
%\backslashbox{$H-V_\ell$}{$H-V_h$}
%&\makebox[3em]{C}&\makebox[3em]{E}\\\hline\hline
%&\makebox[3em]{6/3}&\makebox[3em]{6/4}\\\hline\hline
$H$ & Drawing & $S(x,y,z)$ & Basic unit & Deletion enforcer & Completion enforcer\\\hline\hline
$A_1$ & 
\end{tabular}}
\end{center}
\caption{Gadgets for obtaining incompressibility for graphs in $\mathcal{A}$}
\label{table:cai-table}
\end{table}


==> tables/old/gang.tex <==
\begin{table}
\begin{center}
\scalebox{1}{
\begin{tabular}{| c | c | c | c | c | c | c | c | c | c | c |}
\cline{1-3} \cline{5-7} \cline{9-11}
\# & \textbf{$H$} & \fbox{\textbf{$\overline{H}$}} & & \# & \textbf{$H$} & \textbf{$\overline{H}$} & & \# & \textbf{$H$} & \textbf{$\overline{H}$}\\ \cline{1-3} \cline{5-7} \cline{9-11}
1 & \input{figs/521} & \input{figs/c521} & & 
  8 & \input{figs/543} & \input{figs/c543} & &
    15 & \input{figs/671} & \input{figs/c671} \\ \cline{1-3} \cline{5-7} \cline{9-11}
2 & \input{figs/531} & \input{figs/c531} & &
  9 & \input{figs/551} & \input{figs/c551} & &
    16 & \input{figs/672} & \input{figs/c672} \\ \cline{1-3} \cline{5-7} \cline{9-11}
3 & \input{figs/532} & \input{figs/c532} & & 
  10 & \input{figs/552} & same & & 
    17 & \input{figs/673} & \input{figs/c673} \\ \cline{1-3} \cline{5-7} \cline{9-11}
4 & \input{figs/533} & \input{figs/c533} & & 
  11 & \input{figs/651} & \input{figs/c651} & & 
    18 & \input{figs/791} & \input{figs/c791} \\ \cline{1-3} \cline{5-7} \cline{9-11}
5 & \input{figs/534} & \input{figs/c534} & & 
  12 & \input{figs/661} & \input{figs/c661} & & 
    19 & \input{figs/7101} & \input{figs/c7101} \\ \cline{1-3} \cline{5-7} \cline{9-11}
6 & \input{figs/541} & \input{figs/c541} & & 
  13 & \input{figs/662} & \input{figs/c662} & & 
    20 & \input{figs/8141} & same\\ \cline{1-3} \cline{5-7} \cline{9-11}
7 & \input{figs/542} & \input{figs/c542} & & 
  14 & \input{figs/663} & \input{figs/c663} & & 
    21 & \input{figs/9181} & same\\ \cline{1-3} \cline{5-7} \cline{9-11}
\end{tabular}}
\end{center}
\caption{The base mentioned in Theorem~\ref{thm:to}}
\label{table:gang}
\end{table}


==> tables/old/gist-old.tex <==
\begin{table}
\begin{center}
\scalebox{1}{
\begin{tabular}{|l||*{3}{c|}}\hline
\backslashbox{$H-V_\ell$}{$H-V_h$}
&\makebox[3em]{Complete}&\makebox[3em]{Empty}\\\hline\hline
%&\makebox[3em]{6/3}&\makebox[3em]{6/4}\\\hline\hline
Complete & $\{C_4, H_5\}$ (Lemma~\ref{lem:c-c}) & $\{H_3, H_5, H_{9}, A_{2}, A_{5}, A_{6}, A_{8}, A_{10}\}$ (Lemma~\ref{lem:c-is})\\\hline
Empty & $\emptyset$ (Lemma~\ref{lem:is-c}) & $\{C_4, H_5\}$ (Corollary~\ref{cor:is-is})\\\hline
$P_3$ & $\emptyset$ (Lemma~\ref{lem:small-c}) & $\{C_4, H_1\}$ (Lemma~\ref{lem:small-is})\\\hline
$\overline{P_3}$ & $\emptyset$ (Lemma~\ref{lem:small-c}) & $\emptyset$ (Lemma~\ref{lem:small-is})\\\hline
$P_4$ & $\emptyset$ (Lemma~\ref{lem:small-c}) & $\{H_4\}$ (Lemma~\ref{lem:small-is})\\\hline
claw & $\emptyset$ (Lemma~\ref{lem:small-c}) & $\{H_2\}$ (Lemma~\ref{lem:small-is})\\ \hline
$\overline{\text{claw}}$ & $\emptyset$ (Lemma~\ref{lem:small-c}) & $\emptyset$ (Lemma~\ref{lem:small-is})\\\hline
paw & $\emptyset$ (Lemma~\ref{lem:small-c}) & $\{H_6, A_{4}\}$ (Lemma~\ref{lem:small-is})\\\hline
$\overline{\text{paw}}$ & $\emptyset$ (Lemma~\ref{lem:small-c}) & $\emptyset$ (Lemma~\ref{lem:small-is})\\\hline
diamond & $\{C_4, A_1\}$ (Lemma~\ref{lem:small-c})& $\{H_4, H_7, H_{6}, H_{8}, A_1, A_{9}\}$ (Lemma~\ref{lem:small-is})\\\hline
$\overline{\text{diamond}}$ & $\emptyset$ (Lemma~\ref{lem:small-c}) & $\emptyset$ (Lemma~\ref{lem:small-is})\\\hline
\end{tabular}}
\end{center}
\caption{Gist of Lemmas~\ref{lem:c-c}, \ref{lem:c-is}, \ref{lem:is-c}, \ref{lem:small-c}, \ref{lem:small-is}, and Corollary~\ref{cor:is-is}. The content of a 
  cell corresponds to the graphs $H'$ which \dominates\ $H$, where $H$ is a graph such that $H-V_\ell$ is the graph mentioned in the row and $H-V_h$ is the graph mentioned in the column.}
\label{table:gist}
\end{table}

\begin{comment}
\begin{table}
\begin{center}
\scalebox{1}{
\begin{tabular}{|l||*{3}{c|}}\hline
\backslashbox{$H-V_\ell$}{$H-V_h$}
&\makebox[3em]{Complete}&\makebox[3em]{Empty}\\\hline\hline
%&\makebox[3em]{6/3}&\makebox[3em]{6/4}\\\hline\hline
Complete & $\{C_4, H_5\}$ (Lemma~\ref{lem:c-c}) & $\{H_3, H_5, H_{9}, A_{2}, A_{5}, A_{6}, A_{8}, A_{10}\}$ (Lemma~\ref{lem:c-is})\\\hline
Empty & $\emptyset$ (Lemma~\ref{lem:is-c}) & $\{C_4, H_5\}$ (Corollary~\ref{cor:is-is})\\\hline
$P_3$ & $\emptyset$ (Lemma~\ref{lem:p3-c}) & $\{C_4, H_1\}$ (Lemma~\ref{lem:p3-is})\\\hline
$\overline{P_3}$ & $\emptyset$ (Corollary~\ref{cor:p3b-c}) & $\emptyset$ (Corollary~\ref{cor:p3b-is})\\\hline
$P_4$ & $\emptyset$ (Lemma~\ref{lem:p4-c}) & $\{H_4\}$ (Lemma~\ref{lem:p4-is})\\\hline
claw & $\emptyset$ (Lemma~\ref{lem:claw-c}) & $\{H_2\}$ (Lemma~\ref{lem:claw-is})\\ \hline
$\overline{\text{claw}}$ & $\emptyset$ (Corollary~\ref{cor:clawb-c}) & $\emptyset$ (Corollary~\ref{cor:clawb-is})\\\hline
paw & $\emptyset$ (Lemma~\ref{lem:paw-c}) & $\{H_6, A_{4}\}$ (Lemma~\ref{lem:paw-is})\\\hline
$\overline{\text{paw}}$ & $\emptyset$ (Corollary~\ref{cor:pawb-c}) & $\emptyset$ (Corollary~\ref{cor:pawb-is})\\\hline
diamond & $\{C_4, A_1\}$ (Lemma~\ref{lem:diamond-c})& $\{H_4, H_7, H_{6}, H_{8}, A_1, A_{9}\}$ (Lemma~\ref{lem:diamond-is})\\\hline
$\overline{\text{diamond}}$ & $\emptyset$ (Corollary~\ref{cor:diamondb-c}) & $\emptyset$ (Corollary~\ref{cor:diamondb-is})\\\hline
\end{tabular}}
\end{center}
\caption{Gist of results from Lemma~\ref{lem:c-c} to Corollary~\ref{cor:diamondb-is}. The content of a 
  cell corresponds to the graphs $H'$ which \dominates\ $H$, where $H$ is a graph such that $H-V_\ell$ is the graph mentioned in the row and $H-V_h$ is the graph mentioned in the column. For brevity, some Lemmas/Corollaries are not captured in the Table: for example, Corollary~\ref{cor:is-p3b} is not captured but its \textit{complementary} result (Lemma~\ref{lem:p3-is}) is captured.}
\label{table:gist}
\end{table}
\end{comment}

==> tables/old/gist-small.tex <==
\begin{table}
\begin{center}
\scalebox{1}{
\begin{tabular}{|l||*{5}{c|}}\hline
\backslashbox{$H-V_\ell$}{$H-V_h$}
&\makebox[3em]{$P_3$}&\makebox[3em]{$P_4$}&\makebox[3em]{claw}&\makebox[3em]{paw}&\makebox[3em]{diamond}\\\hline\hline
%&\makebox[3em]{6/3}&\makebox[3em]{6/4}\\\hline\hline
$P_3$ & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$\\\hline
$P_4$ & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$\\\hline
claw & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$\\\hline
paw & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$\\\hline
diamond & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$\\\hline\hline
\backslashbox{$H-V_\ell$}{$H-V_h$}
&\makebox[3em]{$\overline{P_3}$}&\makebox[3em]{$P_4$}&\makebox[3em]{$\overline{\text{claw}}$}&\makebox[3em]{$\overline{\text{paw}}$}&\makebox[3em]{$\overline{\text{diamond}}$}\\\hline\hline
%&\makebox[3em]{6/3}&\makebox[3em]{6/4}\\\hline\hline
$P_3$ & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$\\\hline
$P_4$ & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$\\\hline
claw & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$\\\hline
paw & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\{H_6, A_{3}, A_{7}\}$\\\hline
diamond & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\{H_8\}$\\\hline\hline
\backslashbox{$H-V_\ell$}{$H-V_h$}
& \makebox[3em]{$P_3$} & \makebox[3em]{$P_4$} & \makebox[3em]{claw} & \makebox[3em]{paw} & \makebox[3em]{diamond}\\\hline\hline
%&\makebox[3em]{6/3}&\makebox[3em]{6/4}\\\hline\hline
$\overline{P_3}$ & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$\\\hline
%$P_4$ & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$\\\hline
$\overline{\text{claw}}$ & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$\\\hline
$\overline{\text{paw}}$ & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$\\\hline
$\overline{\text{diamond}}$ & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\emptyset$\\\hline
\end{tabular}}
\end{center}
\caption{Gist of observations leading to Lemma~\ref{lem:small}}
\label{table:gist-small-pp}
\end{table}


==> tables/old/small-is-table.tex <==
\begin{table}
\begin{center}
\scalebox{1}{
\begin{tabular}{|c|c|b{2.2cm}|c|c|c|c|}\hline
Row & Graph & Comment & Dominated by & Comment & Proved by\\\hline
1 & \input{figs/z7101} & see Figure~\ref{fig:z7101} & \input{figs/c4} & $C_4$ & Corollary~\ref{cor:mod}\\\hline
2 & \input{figs/claw-2k1} & & \input{figs/531} & $H_2$ & Corollary~\ref{cor:jutk1} \\\hline
%3 & \input{figs/paw-2k1} & & \input{figs/542} & $H_6$ & Corollary~\ref{cor:jutk1} \\\hline
3 & \input{figs/z7102c} & complement in Figure~\ref{fig:z7102} & \input{figs/534} & $H_4$ & Corollary~\ref{cor:path}, \ref{cor:folklore} \\\hline
4 & \input{figs/z7111} & see Figure~\ref{fig:z7111} & \input{figs/c532} & $\overline{A_1}$ & Corollary~\ref{cor:mod} \\\hline
5 & \input{figs/z9151} & see Figure~\ref{fig:z9151} & \input{figs/z7111} & see row 5 & Corollary~\ref{cor:mod} \\\hline
6 & \input{figs/z8131} & see Figure~\ref{fig:z8131} & \input{figs/c532} & $\overline{A_1}$ & Corollary~\ref{cor:mod} \\\hline
7 & \input{figs/diamond-2k1} & & \input{figs/c551} & $\overline{H_8}$ & Corollary~\ref{cor:mod} \\\hline
8 & \input{figs/671} & complement in Figure~\ref{fig:c671} & \input{figs/c542} & $\overline{H_6}$ & Lemma~\ref{lem:h12}, Corollary~\ref{cor:folklore} \\\hline
9 & \input{figs/z891} & see Figure~\ref{fig:z891} & \input{figs/671} & see row 9 & Corollary~\ref{cor:mod} \\\hline
\end{tabular}}
\end{center}
\caption{Column `Graph' contains all graphs $H$ with at most nine vertices such that $H-V_\ell$ is in $\mathcal{Y'}$, $H-V_h$ is an empty graph, and neither $H$ nor $\overline{H}$ is in $\mathcal{H}\cup\mathcal{A}\cup\mathcal{X}$. See Lemma~\ref{lem:small-is}.}
\label{table:small-is}
\end{table}

==> tables/old/tough-gang.tex <==
\begin{table}
\begin{center}
\scalebox{1}{
\begin{tabular}{| c | c | c | c | c | c | c | c | c | c | c |}
\cline{1-3} \cline{5-7} \cline{9-11}
\# & \textbf{$H$} & \fbox{\textbf{$\overline{H}$}} & & \# & \textbf{$H$} & \textbf{$\overline{H}$} & & \# & \textbf{$H$} & \textbf{$\overline{H}$}\\ \cline{1-3} \cline{5-7} \cline{9-11}
1 & \input{figs/521} & \input{figs/c521} & & 
  4 & \input{figs/534} & \input{figs/c534} & & 
    7 & \input{figs/543} & \input{figs/c543} \\ \cline{1-3} \cline{5-7} \cline{9-11}
2 & \input{figs/531} & \input{figs/c531} & &
  5 & \input{figs/541} & \input{figs/c541} & & 
    8 & \input{figs/551} & \input{figs/c551} \\ \cline{1-3} \cline{5-7} \cline{9-11}
3 & \input{figs/533} & \input{figs/c533} & & 
  6 & \input{figs/542} & \input{figs/c542} & & 
    9 & \input{figs/552} & same\\ \cline{1-3} \cline{5-7} \cline{9-11}
%1 & \input{figs/521} & \input{figs/c521} & & 
%  8 & \input{figs/543} & \input{figs/c543} & &
%    15 & \input{figs/671} & \input{figs/c671} \\ \cline{1-3} \cline{5-7} \cline{9-11}
%2 & \input{figs/531} & \input{figs/c531} & &
%  9 & \input{figs/551} & \input{figs/c551} & &
%    16 & \input{figs/672} & \input{figs/c672} \\ \cline{1-3} \cline{5-7} \cline{9-11}
%3 & \input{figs/532} & \input{figs/c532} & & 
%  10 & \input{figs/552} & same & & 
%    17 & \input{figs/673} & \input{figs/c673} \\ \cline{1-3} \cline{5-7} \cline{9-11}
%4 & \input{figs/533} & \input{figs/c533} & & 
%  11 & \input{figs/651} & \input{figs/c651} & & 
%    18 & \input{figs/791} & \input{figs/c791} \\ \cline{1-3} \cline{5-7} \cline{9-11}
%5 & \input{figs/534} & \input{figs/c534} & & 
%  12 & \input{figs/661} & \input{figs/c661} & & 
%    19 & \input{figs/7101} & \input{figs/c7101} \\ \cline{1-3} \cline{5-7} \cline{9-11}
%6 & \input{figs/541} & \input{figs/c541} & & 
%  13 & \input{figs/662} & \input{figs/c662} & & 
%    20 & \input{figs/8141} & same\\ \cline{1-3} \cline{5-7} \cline{9-11}
%7 & \input{figs/542} & \input{figs/c542} & & 
%  14 & \input{figs/663} & \input{figs/c663} & & 
%    21 & \input{figs/9181} & same\\ \cline{1-3} \cline{5-7} \cline{9-11}
\end{tabular}}
\end{center}
\caption{The set $\mathcal{H}$ of graphs mentioned in Lemma~\ref{lem:to}}
\label{table:tough-gang}
\end{table}
